METAM: Goal-Oriented Data Discovery

Data is a central component of machine learning and causal inference tasks. The availability of large amounts of data from sources such as open data repositories, data lakes and data marketplaces creates an opportunity to augment data and boost those tasks' performance. However, augmentation techniques rely on a user manually discovering and shortlisting useful candidate augmentations. Existing solutions do not leverage the synergy between discovery and augmentation, thus under exploiting data. In this paper, we introduce METAM, a novel goal-oriented framework that queries the downstream task with a candidate dataset, forming a feedback loop that automatically steers the discovery and augmentation process. To select candidates efficiently, METAM leverages properties of the: i) data, ii) utility function, and iii) solution set size. We show METAM's theoretical guarantees and demonstrate those empirically on a broad set of tasks. All in all, we demonstrate the promise of goal-oriented data discovery to modern data science applications.

==> relationship.tex <==
\section{Target Scenarios and Data Profiles\label{sec:targetscenario}}

In this section, we discuss commonly considered downstream tasks along with considered profiles for score estimation.
\subsection{Target Scenario and Downstream Task Implementation}
\label{subsec:tasks}
\sys{} targets scenarios for which analysts can define the task \emph{objective} or \emph{goal} a priori. The goal consists of a downstream task implementation, an initial input dataset ($\din$), and a function to compute the utility achieved by the task when using the input dataset. Then, given the repository of datasets and the goal, \sys{} automatically finds project-join queries that augment $\din$ to boost the downstream task's utility. Many important tasks fit this scenario:

% \mypar{Target Scenario} \sys{} targets scenarios where analysts have access to a dataset, $D$, to perform a downstream task. Analysts want to augment $D$ by combining it with other datasets via project-join queries\footnote{Our framework can consider complex SQL queries over the datasets. We focus on PJ-queries for simplicity and we discuss extensions in Appendix~\ref{?}.} to improve the tasks's quality. The datasets come from possibly very large collection of datasets, such as those found in open data lakes, data warehouses and data lakes within organizations, and even data markets. We present an initial broad set of supported downstream tasks.

% A downstream task is an opaque box that takes a dataset as input and outputs a \emph{utility score} that corresponds to a quality metric that depends on the input dataset. Many important analytic tasks naturally fit this pattern. We explain the tasks we consider in this paper and later, in Section~\ref{subsec:}, we include a discussion on how to extend these.

% \notera{ensure it is clear how the utility score is computed}

\begin{myenumerate}

\item  \textbf{Predictive analytics}: In this category, we consider two types of tasks (i) \textsc{Classification} (ii) \textsc{Regression}. These tasks train a machine learning classifier (or a regression function) over the input dataset to predict a target variable. For example, to predict the \texttt{useful expected life} of wind turbines. In these tasks, the user provides the input dataset $\din$ which contains the target column, and a task implementation that returns a utility score. In its simplest form, the utility score may correspond to accuracy, MAE, or other other complex metrics like fairness, robustness, etc. We refer the reader to Section~\ref{sec:evaluation} for a detailed case study on fair classification.  %metric relevant to the task. \underline{A note on Fairness:} The opaque box may define the utility score so it reflects a \emph{fairness} definition relevant to the task.

\item \textbf{Causal Inference:} We consider \textsc{What-if analysis}, and \textsc{How-to analysis} tasks, which are often found in Business Intelligence products \cite{tableau, powerbi, domo}  widely used by decision makers. First, the \textsc{What-if analysis} task takes an input dataset along with a hypothetical update query, and outputs the causal impact of the update query on other attributes. For example, ``Which attributes are most affected by reducing the \texttt{kWh} capacity of a wind turbine?'' is a query that identifies attributes that are affected causally by the change of the turbine's generation capacity, \texttt{kWh}. To achieve that goal, the task may make use of complex causal inference techniques that test conditional independence among different combinations of attributes to estimate the causal impact, e.g., PC algorithm~\cite{spirtes2000causation}. Second, the \textsc{How-to analysis} task evaluates the causal impact between attributes to solve an optimization problem. For example, ``Which attribute should be updated so that \texttt{useful expected life} stretches 2 more years?''. These systems return the optimization objective or the total causal influence of the updated attribute as the utility score.

\item \textbf{Entity-linking} tasks map entities from a dataset to ontologies and other reference data, such as Wikidata or DBPedia~\cite{dbpedia}. These mappings facilitate searching and recommending data~\cite{galhotra2020semantic}. The task implementation may leverage different attributes along with external sources, such as knowledge graphs and semantic embeddings, to identify entities in a dataset and link them with the ontologies. The task implementation returns the fraction of correctly identified entities as the utility score.

\item \textbf{Cluster Analysis} techniques use attributes of input records to group similar records together (often known as clusters) and infer latent communities in the dataset. Cluster analysis is widely used to mine patterns e.g. community detection in social networks,  gene analysis in biology, anomaly detection, etc. One of the common uses of clustering techniques in data management is to perform entity resolution, which aims to identify clusters of records that refer to the same entity. The task's utility function evaluates accuracy of the identified patterns (or relationships) on a sample of the dataset (often called as the validation set), and returns the accuracy as the utility score. For example, the fraction of record pairs that are correctly labelled as intra-cluster or inter-cluster is commonly used as an evaluation metric to evaluate the clustering output.

\end{myenumerate}



